Digital Social Contracts: A Foundation for an Egalitarian and Just Digital Society

Almost two centuries ago Pierre-Joseph Proudhon proposed social contracts -- voluntary agreements among free people -- as a foundation from which an egalitarian and just society can emerge. A \emph{digital social contract} is the novel incarnation of this concept for the digital age: a voluntary agreement between people that is specified, undertaken, and fulfilled in the digital realm. It embodies the notion of "code-is-law" in its purest form, in that a digital social contract is in fact a program -- code in a social contracts programming language, which specifies the digital actions parties to the social contract may take; and the parties to the contract are entrusted, equally, with the task of ensuring that each party abides by the contract. Parties to a social contract are identified via their public keys, and the one and only type of action a party to a digital social contract may take is a "digital speech act" -- signing an utterance with her private key and sending it to the other parties to the contract. Here, we present a formal definition of a digital social contract as agents that communicate asynchronously via crypto-speech acts, where the output of each agent is the input of all the other agents. We outline an abstract design for a social contracts programming language and show, via programming examples, that key application areas, including social community; simple sharing-economy applications; egalitarian currency networks; and democratic community governance, can all be expressed elegantly and efficiently as digital social contracts.

==> ConcurrentPrologCode/airbnb.tex <==



‪tourist(Self,In,Out) :-‬
‪	tourist(Self,In,Out,roaming).‬

‪tourist(Self,In,Out,roaming) :-‬
‪	true : Out = [reserve(Self)|Out'] | tourist(Self,In,Out',waiting).‬

‪tourist(Self,In,Out,waiting) :-‬
‪	In = [reservation(Self)|In'] : true | tourist(Self,In',Out,lodging).‬

tourist(Self,In,Out,waiting) :-
	In = [reservation_denied(Self)|In'] : true | tourist(Self,In',Out,roaming).


tourist(Self,In,Out,waiting) :-
	In = [_|In'], otherwise : true | tourist(Self,In',Out,waiting).


‪tourist(Self,In,Out,lodging) :-‬
‪	true : Out = [checkout(Self)|Out'] | tourist(Self,In,Out',roaming).‬



‪host(Self,In,Out) :-‬
‪	host(Self,In,Out,free).‬

‪host(Self,In,Out,free) :-‬
‪	In = [reserve(Tourist)|In'] : Out = [reservation(Tourist)|Out'] | 	host(Self,In',Out',reserved(Tourist)).‬

‪host(Self,In,Out,reserved(Tourist)) :-‬
‪	In = [reserve(Tourist1)|In'], Tourist =\= Tourist1 : Out = [reservation_denied(Tourist1)|Out'] | host(Self,In',Out',free).‬

host(Self,In,Out,reserved(Tourist)) :-
	In = [checkout(Tourist)|In'] : true | host(Self,In',Out,free).

host(Self,In,Out,State) :-
	In = [_|In'], otherwise : true | host(Self,In',Out,State).


run(Tourists,Host,History) :-
	tourists(Tourists,History,TOuts),
	host(Host,History,HOut),
	stream#merger([merge(HOut)|TOuts],History).

tourists([T|Ts],History,Outs) :-
	true : Outs = [merge(Out)|Outs'] |
	tourist(T,History,Out),
	tourists(Ts,History,Outs').

tourists([],_,Outs) :- true : Outs = [] | true.



==> smarttable.tex <==

\newcounter{ti}


\newcommand\sti{\addtocounter{ti}{1}\theti}
%\newcommand\sti{\stepcounter{ti}\theti}
%\newcommand\sti{\refstepcounter{ti}\theti}



\begin{flushleft}
\begin{table*}[htp!]
%
%\centering
%

 \begin{tabular}{ | m{14em} || m{16em}| m{16em} | } 
%\begin{tabular}{| m{3em} | m{3em} | m{3em}|} 
 \hline
&   \textbf{Digital Smart Contract} & \textbf{Digital Social Contract}  \\ [2ex] 
 \hline\hline
 \textbf{\sti. Parties (via their public keys)} &  Anonymous Trustless  Accounts & Known Trustworthy People  \\ [2ex]
 \hline
 \textbf{\sti. Party Balance} &  Rights only (never negative) & Rights and Obligations (possibly negative) \\ [2ex]
 \hline
 \textbf{\sti. Enforcement} & Global, Anonymous, Trustless   Miners  &  Local, Known, Trustworthy  Parties  \\[2ex]
 \hline
  \textbf{\sti.  Privacy} &  Public   &  Possibly Private \\ [2ex] 
 \hline
 \textbf{\sti. Utility} & Financial & Social \& Financial  \\[2ex]
 \hline
 \textbf{\sti. Longevity} & Eternal & Up to parties decision  \\[2ex]
 \hline
 
  \textbf{\sti. Amendments  } & Impossible & By parties decision  \\  [2ex]
  \hline
  \textbf{\sti. Recovery from lost or stolen key} & Impossible & By parties decision  \\  [2ex]
  \hline
%  \textbf{\sti. Guardianship, Living Will, Will} & Impossible & By parties cooperation  \\  [2ex]
% \hline
   \textbf{\sti. Multi-Chain Transactions} & Beneficial and complex & Essential and simple  \\  [2ex]
 \hline
\textbf{\sti. Risk} & Byzantine miners majority (Global) &  Byzantine parties supermajority (Local)  \\[2ex] 
\hline
\textbf{\sti. Specification} & Reactive Program &  Distributed Program \\[2ex] 
 \hline
 \textbf{\sti. Implementation} & Globally-Replicated Public Blockchain &   Locally-Replicated Personal Interlocked Blockchains \\[2ex] 
 \hline
 \textbf{\sti. Financial Ecosystem} & Plutocratic, Global Cryptocurrency (e.g. Ethereum) &  Egalitarian Cryptocurrency Network \\[2ex] 
 \hline
 \hline
\end{tabular}
\caption{Digital Smart Contracts vs. Digital Social Contracts}
\label{figure:compare}

\end{table*}
\end{flushleft}

